Geometry of Complex Networks and Topological Centrality

We explore the geometry of complex networks in terms of an n-dimensional Euclidean embedding represented by the Moore-Penrose pseudo-inverse of the graph Laplacian $(\bb L^+)$. The squared distance of a node $i$ to the origin in this n-dimensional space $(l^+_{ii})$, yields a topological centrality index $(\mathcal{C}^{*}(i) = 1/l^+_{ii})$ for node $i$. In turn, the sum of reciprocals of individual node structural centralities, $\sum_{i}1/\mathcal{C}^*(i) = \sum_{i} l^+_{ii}$, i.e. the trace of $\bb L^+$, yields the well-known Kirchhoff index $(\mathcal{K})$, an overall structural descriptor for the network. In addition to this geometric interpretation, we provide alternative interpretations of the proposed indices to reveal their true topological characteristics: first, in terms of forced detour overheads and frequency of recurrences in random walks that has an interesting analogy to voltage distributions in the equivalent electrical network; and then as the average connectedness of $i$ in all the bi-partitions of the graph. These interpretations respectively help establish the topological centrality $(\mathcal{C}^{*}(i))$ of node $i$ as a measure of its overall position as well as its overall connectedness in the network; thus reflecting the robustness of node $i$ to random multiple edge failures. Through empirical evaluations using synthetic and real world networks, we demonstrate how the topological centrality is better able to distinguish nodes in terms of their structural roles in the network and, along with Kirchhoff index, is appropriately sensitive to perturbations/rewirings in the network.

==> Abstract.tex <==
%%%%%%%%%
%
% --- Abstract ---
%
%%%%%%%%%
%
We explore the geometry of complex networks in terms of an n-dimensional Euclidean 
embedding represented by the  Moore-Penrose pseudo-inverse of the graph Laplacian 
$(\bb L^+)$. 
%  
The squared distance of a node $i$ to the origin in this n-dimensional space $(l^+_{ii})$, 
yields a structural centrality index $(\mathcal{C}^{*}(i) = 1/l^+_{ii})$ for node $i$. 
%
In turn, the sum of reciprocals of individual node structural centralities, 
$\sum_{i}1/\mathcal{C}^*(i) = \sum_{i} l^+_{ii}$,  
i.e. the trace of  $\bb L^+$, yields the well-known Kirchoff index $(\mathcal{K})$, 
an overall structural descriptor for  the network. 
%
In addition to this geometric interpretation, we provide alternative interpretations of the 
proposed indices to reveal their true topological characteristics: 
first, in terms of forced detour overheads and frequency of recurrences in random walks 
that has an interesting analogy to voltage distributions in the equivalent electrical network; 
and then as the average connectedness of $i$ in all the bi-partitions of the graph.
% 
These interpretations respectively help establish the structural centrality $(\mathcal{C}^{*}(i))$ 
as a measure of both the overall position as well as the overall connectedness of node $i$ in 
the network which in turn reflects the robustness of node $i$ to random multiple edge failures.
%
Through empirical evaluations using synthetic and real world networks, we demonstrate how the 
structural centrality is better able to distinguish nodes in terms of their structural roles in the network 
and, along with Kirchoff index, is appropriately sensitive to perturbations/rewirings in the network. 
%
%%%%%%%%%%%
%
% --- End Abstract ---
%
%%%%%%%%%%%


==> Conclusion.tex <==
%%%%%%%%%%
%
% --- Conclusion ---
%
%%%%%%%%%%
%
In this work, we presented a geometric perspective on robustness in complex  
networks in terms of the Moore-Penrose pseudo-inverse of the graph Laplacian. 
We proposed structural centrality $(\mathcal{C}^*(i))$ and Kirchoff 
index $(\mathcal{K}(G))$ that respectively reflect the length of the position vector 
for a node and the overall volume of the graph embedding and therefore are 
suitable geometric measures of robustness of individual nodes and the overall network. 
Additionally, we provided interpretations for these indices 
in terms of the overhead incurred in random detours through a node in question 
as well as in terms of the recurrence probabilities and voltage distribution in the 
EEN corresponding to the network. Both indices reflect the global connectedness 
properties of individual nodes and the network on a whole, particularly in the event 
of multiple edge failures that may render the network disconnected. 
Through numerical analysis on simulated and real world networks, we demonstrated 
that $\mathcal{C}^*(i)$ captures structural roles played by nodes in networks and, 
along with Kirchoff index, is suitably sensitive to perturbations/rewirings in 
the network. In terms of computational complexity, structural centrality 
compares well with other geodesic and all-paths based indices in literature 
(see Table \ref{tab:Taxonomy}) and performs better than random-walk betweenness 
in the asymptotic case. 
%
In future, we aim at investigating similar metrics for the case of 
strongly connected weighted directed graphs to further generalize our work.  
%
%
\begin{table}
\caption{Taxonomy and computational complexities of centrality measures (for all nodes).}
\label{tab:Taxonomy}
\centerline{
\begin{tabular}
{|c|l|c|c|}
\hline
\# & Measure & Paths covered & Complexity \\
\hline \hline
1. & Degree & - & $O(m)$\\
\hline
2. & $GC$,  $GB$ & Geodesic paths & $O(n^3)$\\
%
\hline\hline
%
3. & $\mathcal{C}^*$ & All paths & $O(n^3)$\\
%
\hline
%
4. & $SC$ & All paths & $O(n^3)$\\
%
\hline
%
5. & $RWB$  & All paths & $O(m + n) n^2$\\ 
%
\hline
%
6. & $FB$ & All paths & $O(m^2 n)$ \\
\hline
\end{tabular}}
\end{table}
%
%%%%%%%%%%%
%
% --- End Abstract ---
%
%%%%%%%%%%%


==> Section_1_Introduction.tex <==
%%%%%%%%%%%
%
% --- Introduction ---
%
%%%%%%%%%%%
%
Unlike traditional studies on network robustness, that typically treat 
networks as combinatoric objects and rely primarily on classical 
graph-theoretic concepts (e.g. minimum cuts), we explore a geometric 
approach which enables us to employ more advanced theories and 
techniques. More importantly, such an approach helps quantify and compare 
robustness of different nodes in the same network as well as different networks 
of comparable sizes, in terms of their local and global structures. 
%

In this work, we study a geometric embedding of networks using the 
Moore-Penrose (pseudo) inverse of the graph Laplacian for the network, 
denoted henceforth by $\bb L^{+}$. We show that the diagonal entries of 
$\bb L^{+}$, denoted as $l^+_{ii}$ for node $i$, that represent 
the squared distance of each node to the origin in the $n-dimensional$ 
Euclidean space of the network embedding, provide 
a robust measure of a node's structural centrality, given as 
$\mathcal{C}^{*}(i) = 1/l^+_{ii}$.
%
In particular, closer a node $i$ is to the origin in this space, more structurally 
central it is. 
%
Moreover, the trace of $\bb L^{+}$, $Tr(\bb L^{+}) = \sum_i 1/\mathcal{C}^{*}(i)$, 
yields the {\em Kirchoff index} $(\mathcal{K})$, a structural descriptor for the network 
as a whole.
% 
Once again, lower the value of $\mathcal{K}$ for a network, more compact the 
embedding, and more structurally robust the overall network is.
%

In addition to the geometric interpretation of structural centrality and Kirchoff 
index described above, we provide three alternative interpretations which 
respectively show how $\mathcal{C}^*(i)$ quantifies the overall position and 
connectedness of a node $i$, and therefore its robustness to failures in the network.
We describe each of these separately below. 
% 

First, we equate structural centrality of a node $i$,  i.e. $\mathcal{C}^*(i)$, 
to the (reciprocal of) average detour overhead incurred when a random walk between 
any source destination pair is forced to go through node $i$. Intuitively, the 
average overhead incurred in such detours (measured in terms of the number 
of steps in the random walk) will be lower if node $i$ is structurally central 
(higher  $\mathcal{C}^*(i)$ and lower $l^+_{ii}$) and vice versa. 
%

Secondly, we show how $\mathcal{C}^*(i)$ is related to electrical voltages when 
the network is treated as an equivalent electrical network (EEN). This, in turn, yields 
an interpretation of $\mathcal{C}^*(i)$ in terms of the probability with which a random 
detour through $i$ returns to the source node; referred to as the phenomenon of 
{\em recurrence} in random walk literature. More precisely, higher $\mathcal{C}^*(i)$ 
implies that a random detour through node $i$ forces the random walk between any 
source destination pair to return to the source node with lower probability, 
thereby incurring lower detour overhead. Both of these interpretations, namely average 
detour overhead and probability of recurrence, show how $\mathcal{C}^*(i)$ quantifies 
the overall position of node $i$ in the network. 
%

Last but not the least, we establish how $\mathcal{C}^*(i)$ captures the overall connectedness 
of node $i$. To do so, we equate it to the number of nodes that $i$ can communicate with when 
a sub-set of edges in the network fail in such a way that the network is partitioned into two connected 
sub-networks. 
%
A higher value of $\mathcal{C}^*(i)$, implies that $i$ is present in the larger of the two 
sub-networks, on an average, resulting from such partitioning. In other words, $\mathcal{C}^*(i)$ reflects 
the immunity/vulnerability of node $i$ towards multiple edge failures in the network, a distinct topological 
characteristic. 
%

Through numerical simulations using synthetic and realistic network topologies, 
we demonstrate that our new indices better characterize robustness of nodes in 
network, both in terms of position as well as connectedness, as compared to other existing metrics 
(e.g. node centrality measured based on degree, shortest paths, etc.). 
A rank-order of nodes in terms of their structural centralities helps distinguish them 
in terms of their structural roles (such as core, gateway, etc.). Also, structural centrality and  
Kirchoff index, are both appropriately sensitive to local perturbations in the network, a 
property not displayed by other centralities in literature (as shown later in this paper).
%

The rest of the paper is organized as follows:   
%
we begin by providing a brief overview of several structural indices, characterizing node centrality 
as well as overall descriptors for networks, found in literature in \textsection\ref{sec:RelWork}.
%
\textsection\ref{sec:Geometry} introduces  a geometric embedding of  the network using the eigen-space 
of $\bb L^+$, structural centrality and Kirchoff index as measures of robustness.
%
\textsection\ref{sec:StructCentAndRandomWalks} demonstrates how  structural centrality of a 
node reflects the average detour overhead in random walks through a particular node in question followed 
by its equivalence to the probability of recurrence.
%  
In \textsection\ref{sec:Partitions} we show how structural centrality captures the average connectedness of  nodes in the bi-partitions of a network. 
%
\textsection\ref{sec:Empirical} presents comparative empirical analysis  
and in \textsection\ref{sec:Conclusion} the paper is concluded.
%
%%%%%%%%%%%%%
%
% --- End Introduction ---
%
%%%%%%%%%%%%%


==> Section_2_RelWork.tex <==
%%%%%%%%%%%
%
% --- Introduction ---
%
%%%%%%%%%%%
%
Robustness of  nodes to failures in complex networks is dependent on their 
overall {\em position} and {\em connectedness} in the network.
%
Several centralities, that characterize position and/or connectedness of nodes 
in complex networks in different ways, have therefore been proposed in literature.
% 
Perhaps the simplest of all is degree --- the number of edges incident on a node. 
Degree is essentially a {\em local} measure i.e. a first oder/one-hop connectedness index. 
%
A second-order variant called {\em joint-degree}, 
given by the product of degrees of a pair of nodes that are connected by an edge in the 
network, is also in vogue. However, except in {\em scale free} networks that display the 
so called {\em rich club connectivity} \cite{Barabasi00, Faloutsos99, Barabasi01}, 
neither degree nor joint-degree determine the overall position or the connectedness of nodes.
%

A class of structural indices called {\em betweennesses}, namely shortest path/geodesic $(GB)$
\cite{Freeman77, Freeman79}, flow $(FB)$ \cite{Freeman91} and random-walk $(RB)$ 
\cite{Newman05} betweenness respectively quantify the positions of nodes, with 
respect to source destination pairs in the network. Betweennesses reflect the role played by a 
node in the communication between other nodes and are not the measures of a node's own 
connectedness. 
% 

A more sophisticated measure is geodesic closeness $(GC)$\cite{Freeman77, Freeman79}. 
It is defined as the (reciprocal of) average shortest-path distance of a node from all other nodes 
in the network. Clearly, geodesic closeness is a $p^{th}$-order measure of connectedness 
where $p = \{1, 2, ..., \delta\}$, $\delta$ being the geodesic diameter of the graph, and is better 
suited for characterizing global connectedness properties than the aforementioned indices.
% 
However, communication in networks  is not always confined to shortest paths alone and $GC$ 
being geodesic based, ignores other alternative paths between nodes, however competitive they 
might be, and thus only partially captures connectedness of nodes. Some all paths based 
counterparts of geodesic closeness include information centrality \cite{Stephenson89} and 
random-walk centrality \cite{Noh04}, that use random-walk based approach to measure centrality.   
%

Recently, subgraph centrality $(SC)$ --- the number of subgraphs of a graph that a node 
participates in --- has also been proposed \cite{Estrada05}. In principle, a node with high 
subgraph centrality, should be better connected to other nodes in the network through 
redundant paths. 
% 
Alas, subgraph centrality is computationally intractable and the proposed 
index in \cite{Estrada05} approximates subgraph centrality by the sum of lengths of all 
{\em closed} walks, weighed in inverse proportions by the factorial of their lengths.
This inevitably results in greater correlation with node degrees as each edge contributes 
to closed random-walks of lengths $2, 4, 6, ...$  and thus introduces local connectivity bias. 
In a subsequent paper, Estrada et al introduce the concept of vibrations to measure node 
vulnerability in complex networks \cite{Estrada10}. Their index called {\em node displacement} 
bears significant resemblance to information centrality and has interesting analogies to physical 
systems. However, once again the true topological significance of the centrality measure, 
in terms of connectedness is wanting. 
%

Our aim in this work, therefore, is to provide an index for robustness of 
nodes in complex networks,  that effectively reflects both the position and connectedness 
properties of nodes and consequently, by extension, of the overall network. 
%
%
%%%%%%%%%%%%%
%
% --- End Introduction ---
%
%%%%%%%%%%%%%


==> Section_3_Geometry.tex <==
%%%%%%%%
%
% --- Section ---
%
%%%%%%%%
%
In studying the {\em geometry} of networks, we first need to embed a network 
(e.g. represented abstractly as a graph) into an appropriate geometric 
space endowed with a metric function (mathematically, a metric space). In this 
section we describe an n-dimensional embedding of the complex network using, 
the Moore-Penrose pseudo-inverse of the combinatorial laplacian $(\bb L^{+})$. 
The squared length of the position vector for a node in this space yields a geometric 
measure of centrality for the node while the sum of the squared lengths of the 
position vectors of all nodes, or the trace of $\bb L^{+}$, yields an overall robustness 
index for the graph. But first  we need to introduce some basic notations. 
%

Given a complex network, its topology is in general represented as a (weighted) 
graph, $G = (V,E,W)$, where $V(G)$ is the set of nodes representing, say, switches, 
routers or end systems in the network; $E = \{e_{uv} : u, v \in V \}$ is the set of edges 
connecting pairs of nodes representing, for example, the (physical or logical) 
communication links between the pair of nodes; and 
$W = {w_{uv} \in \Re^{+} : e_{uv} \in E(G)}$ is a set of weights assigned to each 
edge of the graph (here $\Re^{+}$ denotes the set of nonnegative real numbers). 
These weights can be used to represent, for example, the capacity, latency, or 
geographical distance, or an (administrative) routing cost associated with the edge 
(communication link) $e_{uv}$. Note that if $w_{uv}$ is simply $0$ or $1$, we have 
a simple and unweighted graph.
%

Given $G = (V, E, W)$, we introduce an $n \times n$ {\em affinity} matrix 
$\bb A = [a_{ij}]$ associated with $G$, where $n = |V(G)|$ is the number of nodes 
in $G$ (the {\em order} of G), and $a_{ij} \geq 0$ is some function of the weight 
$w_{ij}$. For a simple graph where $w_{ij} \in \{0, 1\}$, setting $a_{ij} = w_{ij}$ 
yields the standard adjacency matrix of the graph $G$. In general, each entry 
$a_{ij}$ captures some measure of affinity between nodes $i$ and $j$: the larger 
$a_{ij}$ is, nodes $i$ and $j$ are in a sense {\em closer} or more {\em strongly connected}. 
Hence in general, we refer to $\bb A$ as an affinity matrix associated with $G$. 
We assume that $a_{ij} = a_{ji}$, i.e. $\bb A$ is symmetric. For $1\leq i \leq n$, define 
$d(i) = \sum_{j} a_{ij}$, and refer to $d(i)$ as the (generalized) degree of node 
$i$. (Note that if $G$ is a simple unweighted graph $j$ and $\bb A$ is its adjacency 
matrix, then $d(i)$ is the degree of node $i$.)
%

The {\em combinatorial Laplacian} of $\bb A$ (or the associated graph $G$), is defined 
as $\bb L = \bb D - \bb A$, where $\bb D = [d_{ii}] = d(i)$ is a diagonal matrix with 
$d(i)$'s on the diagonal. The Laplacian is a positive semidefinite matrix, and thus 
has $n$ non-negative Eigen values $\lambda_{i}$'s. For $1 \leq i \leq n$, let 
$\bb u_{i}$ be the corresponding eigenvector of $\lambda_{i}$ such that 
$||\bb u_i||_2^2 = \bb u_{i}' \bb u_{i}$. We assume that the eigenvalues 
$\lambda_i$'s are ordered such that $\lambda_1\geq ... \geq \lambda_n = 0$. 
Then the matrix formed by the corresponding eigenvectors $\bb u_{i}'s$, 
$\bb U = [\bb u_1, ..., \bb u_n ]$, is orthogonal i.e. $\bb U' \bb U = \bb I$, the 
identity matrix. More importantly, $\bb L$ admits an eigen decomposition 
$\bb L = \bb U \Lambda \bb U'$, where $\Lambda$ is the diagonal matrix 
$\Lambda = [\lambda_{ii}] = \lambda_i$. 
% 

Like $\bb L$, its Moore-Penrose (pseudo) inverse $\bb L^+$ is also positive semi-definite, 
and admits an eigen decomposition of the form, $\bb L^+ = \bb U \Lambda^{+} \bb U'$, 
where $\bb \Lambda^{+}$ is a diagonal matrix consisting of $\lambda^{-1}$ if $\lambda_i > 0$, 
and 0 if $\lambda_i = 0$ (for simplicity of notation, in the following we will use the 
convention $\lambda^{-1}_i= 0$ if $\lambda_i = 0$). Define $\bb X = \Lambda^{+1/2} \bb U'$. 
Hence, $\bb L^{+} = \bb X' \bb X$ which means that the network can be embedded into the 
Euclidean space $\Re^n$ where the coordinates of node $i$ are given by $\bb x_i$, the $i^{th}$ 
column of $\bb X$.
% 
As the centroid of the position vectors lies at the origin in this n-dimensional space \cite{Fouss07},  
the squared distance of node $i$ from the origin is exactly the corresponding diagonal entry of 
$\bb L^+$ i.e. $||\bb x_i||^2_2 = l^+_{ii}$ and the squared distance between two nodes 
$i, j \in V(G), ||\bb x_i - \bb x_j||^2_2 = Vol(G)^{-1} C_{ij}$ where $Vol(G) = \sum_{i=1}^n d(i)$  
is called the {\em volume} of the graph (a constant for the graph) and $C_{ij}$ is called the 
{\em commute time} defined as the expected length of commute in a random walk between $i$ 
and $j$ in the network \cite{Chandra89}. 
%

Based on the geometric embedding of the graph using $\bb L^+$ described above, we now put 
forth two robustness metrics. First, a rank order for individual nodes in terms of their relative 
robustness called {\em structural centrality}, defined as: 
%
\begin{mydef}
%
Structural centrality of node $i \in V(G)$: 
%
\begin{equation}
%
\mathcal{C}^*(i) = 1/l^+_{ii}, ~~~ \forall i \in V(G) 
%
\end{equation}
%
\end{mydef}
%
Specifically, closer a node is to the origin in this n-dimensional space, more 
structurally central it is and consequently greater its robustness (as shown later). 
%
Next, a structural descriptor for the overall robustness of the network called {\em Kirchoff index}, 
defined as:
%
\begin{mydef}
%
Kirchoff index for $G(V, E)$: 
%
%
\begin{equation}
%
\mathcal{K}(G) = Tr(\bb L^+) = \sum_{i=1}^n l^+_{ii} = \sum_{i=1}^n 1/ \mathcal{C}^*(i)
%
\end{equation}
%
\end{mydef}
%
Geometrically, more compact the embedding is, lower the value of $\mathcal{K}(G)$ and 
more robust the network $G$ is. It is worth pointing out that Kirchoff index has been used to 
model molecular strengths in the theoretical chemistry literature \cite{Xiao03}, primarily because 
it has interesting analogies in the field of electrical networks but its true topological significance 
has scarcely been explored previously.  Also, since 
 
\begin{equation}
\mathcal{K}(G) = Tr(\bb L^+) = \sum_{i=1}^{n-1} \frac{1}{\lambda_i}
\end{equation}

\noindent Kirchoff index can be thought of as a more generalized version of the much celebrated 
{\em algebraic connectivity} of the graph, measured by the second smallest eigen-value 
of the Laplacian i.e. $\lambda_{n-1}$ \cite{Fiedler73, Fiedler75}.
%
We can therefore use Kirchoff index to compare the robustness of two 
graphs with the same order and volume.       

In what follows, we demonstrate how these two metrics indeed reflect robustness of nodes and the 
overall graph respectively, first through rigorous mathematical analysis resulting in closed form 
representations and  then with empirical evaluations over realistic network topologies.
%
%
%%%%%%%%%%%
%
% --- End Section ---
%
%%%%%%%%%%%


==> Section_4_StructCentAndRandomWalks.tex <==
%%%%%%%%
%
% --- Section ---
%
%%%%%%%%
% 
To show that structural centrality $(\mathcal{C}^*(i))$ indeed captures the overall position of a node, 
we relate it to the lengths of random-walks on the graph.
% 
In \textsection\ref{subsec:Detour}, we demonstrate how $\mathcal{C}^*(i)$ is related to the average  
overhead incurred in random {\em detours} through node $i$ as a {\em transit} vertex. 
%
Next in \textsection\ref{subsec:RecurVoltAndElectNet}, we provide an electrical interpretation for it in terms 
of voltages and the probability with which a random detour through node $i$ returns to the source node. 
%
%
\subsection{Detours in Random Walks}
\label{subsec:Detour}
%
A simple random walk $(i \rightarrow j)$, is a discrete stochastic process 
that starts at a node $i$, the source, visits other nodes in the graph $G$ 
and stops on reaching the destination $j$  \cite{GobelJagers74}. In contrast, 
we define a {\em random detour} as:
%
\begin{mydef}
Random Detour $(i \rightarrow k \rightarrow j)$: A random walk starting from 
a source node $i$, that must visit a transit node $k$, before it reaches the 
destination $j$ and stops.
%
\end{mydef}
%
Effectively, such a random detour is a combination of two simple random walks: 
$(i \rightarrow k)$ followed by $(k \rightarrow j)$. We quantify the difference 
between the random detour $(i \rightarrow k \rightarrow j)$ and the simple random 
walk $(i \rightarrow j)$ in terms of the number of steps required to complete 
each of the two processes given by hitting time.
%
\begin{mydef}
Hitting Time $(H_{ij})$: The expected number of steps in a 
random walk starting at node $i$ before it reaches node $j$ for the first 
time. 
\end{mydef}
%
Clearly, $H_{ik} + H_{kj}$ is the expected number of steps in the random 
detour $(i \rightarrow k \rightarrow j)$. Therefore, the overhead incurred is: 
%
%
\begin{equation}
%
\Delta H^{i \rightarrow k \rightarrow j}  = H_{ik} + H_{kj} - H_{ij}
\label{equ:DetOverhead}
%
\end{equation}
%
Intuitively, more peripheral transit $k$ is, greater the overhead in (\ref{equ:DetOverhead}). 
The overall peripherality of $k$ is captured by the following average:
%
\begin{equation}
%
\Delta H^{(k)}
= \frac{1}{n^2 ~Vol(G)} 
\sum_{i = 1}^{n} \sum_{j = 1}^{n} \Delta H^{i \rightarrow k \rightarrow j}
% 
\label{equ:RandEcc}
%
\end{equation}
%
Alas, hitting time is not a Euclidean distance as $H_{ij} \neq H_{ji}$ 
in general. An alternative is to use commute time 
$C_{ij} = H_{ij} + H_{ji} = C_{ji}$, a metric, instead. More importantly \cite{KleinRandic93}, 
%
\begin{equation}
%
C_{ij} = Vol(G) (l^+_{ii} + l^+_{jj} - l^+_{ij} - l^+_{ji})
%
\end{equation}
%
and in the overhead form $(\ref{equ:DetOverhead})$, (non-metric) hitting and 
(metric) commute times are in fact equivalent 
(see propositions $9-58$ in \cite{Kemeny66}):
%
\begin{equation}
%
\Delta H^{i \rightarrow k \rightarrow j} = (C_{ik} + C_{kj} - C_{ij})/2 
= \Delta H^{j \rightarrow k \rightarrow i}
%
\end{equation}
% 
We now exploit this equivalence to equate the cumulative detour overhead 
through transit $k$ from (\ref{equ:RandEcc}) to $l^+_{kk}$ in the following 
theorem.\newline
%
%
%%%%%%%%%%
% Theorem
%%%%%%%%%%
%
%
\noindent\begin{mythm} \label{thm:RandEccLp}
%
\begin{equation}
%
\Delta H^{(k)} = l^+_{kk}
%
\end{equation}
%
\end{mythm}
%
\textbf{Proof:}
Using $\Delta H^{i \rightarrow k \rightarrow j} = (C_{ik} + C_{kj} - C_{ij})/2$:
%
\begin{eqnarray*}
%
\Delta H^{(k)} &=& 
%
\frac{1}{2 n^2  ~Vol(G)} 
\sum_{i = 1}^{n} \sum_{j = 1}^{n} C_{ik} + C_{kj} - C_{ij}
%
%
\end{eqnarray*}
%
Observing $C_{xy}= Vol(G)~(l^{+}_{xx} + l^{+}_{yy}- 2 l^{+}_{xy})$ 
\cite{KleinRandic93} and that $\bb L^+$ is doubly centered 
(all rows and columns sum to $0$) \cite{Fouss07}, we obtain the proof.
%

\noindent $\square$
%

\noindent Therefore, a low value of $\Delta H^{(k)}$ implies higher $\mathcal{C}^*(k)$ and more 
structurally central node $k$ is in the network. Theorem \ref{thm:RandEccLp} is interesting for 
several reasons. First and foremost, note that:
%
\begin{equation}
%
\sum_{j=1}^{n} C_{kj} = Vol(G) ~(n~ l^{+}_{kk} + Tr(\bb L^+))
%
\end{equation}
% 
As $Tr(\bb L^+)$ is a constant for a given graph and an invariant with 
respect to the set $V(G)$, we obtain 
$l^+_{kk} \propto \sum_{j=1}^{n} C_{kj}$;  
lower $l^+_{kk}$ or equivalently higher $\mathcal{C}^*(k)$, implies shorter 
average commute times between $k$ and the rest of the nodes in the graph 
on an average. 
%
Moreover,
%
\begin{equation}
%
\mathcal{K}(G) = Tr(\bb L^+)=\sum_{k = 1}^n l^+_{kk} = \frac{1}{2n Vol(G)} \sum_{k=1}^{n}\sum_{j=1}^{n} C_{kj}
%
\end{equation} 
% 
As $\mathcal{K}(G)$ reflects the average commute time between any pair of nodes in the network, 
it is a measure of overall connectedness in $G$. For two networks of the same order $(n)$ and 
volume $(Vol(G))$, the one with lower $\mathcal{K}(G)$ is better connected on an average. 
%
%
\subsection{Recurrence, Voltage and Electrical Networks}
%
\label{subsec:RecurVoltAndElectNet}
%
%
Interestingly, the detour overhead in  $(\ref{equ:DetOverhead})$ is related 
to {\em recurrence} in random walks --- the expected number of times a 
random walk  $(i \rightarrow j)$ returns to the source $i$  \cite{DoyleSnell84}. 
We now explore how recurrence in detours related to structural centrality 
of nodes. But first we need to introduce some terminology.
%

The equivalent electrical network (EEN)  \cite{DoyleSnell84} for $G(V, E, W)$ 
is formed by replacing an edge $e_{ij} \in E(G)$ with a resistance equal to 
$w_{ij}^{-1}$ (see Fig. \ref{fig:GraphEEN}). The {\em effective resistance} 
($\Omega_{ij}$) is defined as the voltage developed across a pair of terminals 
$i$ and $j$ when a unit current is injected at $i$ and is extracted from $j$, 
or vice versa.
%
%
In the EEN, let $V^{ij}_{k}$ be the voltage of node $k$ when a unit current is 
injected at $i$ and a unit current is extracted from $j$. From \cite{Tetali91}, 
$U^{ij}_{k} = d(k) V^{ij}_{k}$.
%
Substituting $k=i$ we get, $U^{ij}_i = d(i) V^{ij}_i$; the expected number of 
times a random walk  $(i \rightarrow j)$ returns to the source $i$. For a finite 
graph $G$, $U^{ij}_i > 0$.
%
%
\begin{figure}[t]
\centerline{\begin{tabular}{c}
%
%
\scalebox{0.8}{\includegraphics[width = 100mm]{graph_EEN.eps}}
%
\end{tabular}}
\caption{A simple graph $G$  and its EEN.}
\label{fig:GraphEEN}
\end{figure}
%
%
The following theorem connects recurrence to the 
detour overhead. 
%
\begin{mythm} \label{thm:DetOverheadRetCount}
%
\begin{eqnarray*}
%
\Delta H^{i \rightarrow k \rightarrow j} 
&=& \frac{Vol(G) ~ (U^{ik}_{i} + U^{kj}_{i} - U^{ij}_{i})}{d(i)}
\\
&=&
Vol(G) ~ (V^{ik}_{i} + V^{kj}_{i} - V^{ij}_{i})
%
\end{eqnarray*}
%
\end{mythm}
%
\textbf{Proof:} From \cite{Tetali91} we have, 
$\Delta H^{i \rightarrow k \rightarrow j} = d(i)^{-1} ~Vol(G) ~ U^{jk}_i$. 
The rest of this proof follows by proving 
$U^{jk}_{i} = U^{ik}_{i} + U^{kj}_{i} - U^{ij}_{i}$.
%

From the \textit{superposition principle} of electrical current, 
we have $V^{xz}_{x} = V^{xz}_{y} + V^{zx}_{y}$. Therefore,
% 
\begin{eqnarray*}
V^{ik}_{i} + V^{kj}_{i} - V^{ij}_{i}   
&=& 
V^{ik}_{j} + V^{ki}_{j} +  V^{kj}_{i} - V^{ij}_{k} + V^{ji}_{k}
\\
&=&
V^{ik}_{j} + (V^{ki}_{j} +  V^{kj}_{i} - V^{ij}_{k} - V^{ji}_{k}) 
\end{eqnarray*}
%
%
From the \textit{reciprocity principle}, $V^{xy}_{z} = V^{zy}_{x}$. Therefore,
%
$V^{ik}_{i} + V^{kj}_{i} - V^{ij}_{i}  = V^{jk}_{i}$.
%
%
Multiplying by $d(i)$ on both sides we obtain the proof.

\noindent $\square$
%

The term $(U^{ik}_{i} + U^{kj}_{i}) - U^{ij}_{i}$ can be interpreted as the expected 
extra number of times a random walk returns to the source $i$ in the random 
detour $(i \rightarrow k \rightarrow j)$ as compared to the simple random 
walk $(i \rightarrow j)$. 
%
Each instance of the random process that returns to the source, 
must effectively start all over again. Therefore, more often the walk returns 
to the source greater the expected number of steps required to complete the 
process and less central the transit $k$ is, with respect to the source-destination 
pair $(i, j)$.

Therefore, $\Delta H^{(k)}$, that is the average of $\Delta H^{i \rightarrow k \rightarrow j}$ 
over all source destination pairs, tells us the average increase in recurrence caused 
by node $k$ in random detours between any source destination pair in the network. 
Higher the increase in recurrence, i.e. $\Delta H^{(k)}$, lower the magnitude of 
$\mathcal{C}^*(k)$ and less structurally central the node $k$ is in the network. 
% 
%
%%%%%%%%%%%
%
% --- End Section ---
%
%%%%%%%%%%%



==> Section_5_Partitions.tex <==
%
%##############
%
% ----- Section -----
%
%##############
%
%
\begin{figure}
\centerline{\begin{tabular}{cc}
%
%
\scalebox{0.75}{\includegraphics[width = 40mm]{graph_Partition.eps}}
&
\scalebox{0.75}{\includegraphics[width = 40mm]{graph_ForestPartition.eps}}
\\
%
(a) Partition $P=(S,S')$ & (b) Spn. forest in $P=(S,S')$
\\
%
%
\end{tabular}}
\caption{Partitions and spanning forests of a graph.}
\label{fig:CutPartition}
\end{figure}
%
Having established, that nodes with higher $\mathcal{C}^*(i)$, 
are more structurally central in the network, we now turn to average connectedness 
of nodes in this section. To show how structural centralities of nodes capture their 
immunity/vulnerability to random failures in the network, we study their connectedness 
in all the bi-partitions of a graph.
%
\begin{mydef}
%
Bi-partition $(P=(S, S'))$: A cut of the graph $G$ which contains exactly two 
mutually exclusive and exhaustive connected subgraphs $S$ and $S'$.
%
\end{mydef}
%
Let, $V(S)$ and $V(S')$ be the mutually exclusive and exhaustive subsets of 
$V(G)$, $E(S)$ and $E(S')$, the sets of edges in the respective components 
$S$ and $S'$ of $P$ and $E(S, S')$, the set of edges that violate $P$ i.e. have 
one end in $S$ and the other in $S'$.
% 
Also, let $\mathcal{T}(S)$ and $\mathcal{T}(S')$ be the set of spanning trees 
in the respective component sets $S$ and $S'$.
% 
We denote by $\mathcal{P}(G)$, the set of all bi-partitions of $G(V, E)$. 
Clearly, a given $P=(S, S')$ represents a state of the network in which $E(S, S')$ 
have failed. A node $i \in V(S)$ stays connected to $|V(S)| - 1$ nodes 
and gets disconnected from $|V(S')|$ nodes.
% 
In the following relationship we show how structural centrality of node $i$ is related to a  
weighted sum of $|V(S)'|$ over all the bi-partitions $P \in \mathcal{P}(G)$ of the network.
%
\begin{mythm}
%
\label{thm:LpPropPartitions}
%
\begin{equation}
%
l^+_{ii} \propto \sum_{P \in \mathcal{P}(G)}^{i \in V(S)} |\mathcal{T}(S)| |\mathcal{T}(S')| |V(S')|
%
\end{equation}
%
\end{mythm}
%
\textbf{Proof sketch:} The following result, due to Chebotarev et al.  \cite{ChebShamis97, ChebShamis98b}, 
forms the basis of our proof. Let $\mathcal{F}_{x}$ be the set of spanning rooted forests of $G(V, E)$ with 
$x$ edges. Precisely, $F_{x} \in \mathcal{F}_{x}$, is a spanning acyclic subgraph of $G$ with the same node 
set as $G$ and is composed of exactly $n - x$ trees with one node marked as a {\em root} in each of 
these $x$ trees. Let $\mathcal{F}^{ii}_{x}$, be the subset of $\mathcal{F}_{x}$ in which node $i$ is the root 
of the tree in which it belongs. Then,
%
\begin{equation}
%
\label{equ:DenseSRFs}
%
l^+_{ii} 
= \frac{\varepsilon(\mathcal{F}^{ii}_{n-2}) - \frac{1}{n} \varepsilon(\mathcal{F}_{n-2})}
{\varepsilon(\mathcal{F}_{n-1})}
%
\end{equation}
%
Here, $\varepsilon(\cdot)$ simply represents the cardinality of the input set 
(see  \cite{ChebShamis97, ChebShamis98b} for details).  
Clearly,  $\varepsilon(\mathcal{F}_{n-2})$ and  $\varepsilon(\mathcal{F}_{n-1})$ 
are invariants over the set of vertices $V(G)$ for a given graph.
% 
Hence, $l^+_{ii} \propto \varepsilon(\mathcal{F}^{ii}_{n-2})$.
%
The rest of the proof follows from the results of the following lemmas:
%
\begin{mylem} 
\label{lem:RandEccPerPartition}
%
Let $\mathcal{F}^{ii}_{n - 2|P}$ be the set of spanning forests with 
$n - 2$ edges (or exactly two trees) rooted at node $i$ in a given bi-partition $P=(S, S')$ and 
$\mathcal{T}_S$, $\mathcal{T}_{S'}$ be the set of spanning trees in $S$ and 
$S'$ respectively. If $i \in V(S)$ then,
%
$$\varepsilon(\mathcal{F}^{ii}_{n - 2|P}) = |\mathcal{T}_S| ~ |\mathcal{T}_{S'}| ~ |V(S')|$$ 
%
\end{mylem}
%
\textbf{Proof :} Let $T_1 \in \mathcal{T}_S$ and $T_2 \in \mathcal{T}_{S'}$. 
Clearly, $|E(T_1)| = |V(S)| - 1$ and $|E(T_2)| = |V(S')| - 1$. 
As $|V(S)| + |V(S')| = |V(G)|$ and $|E(T_1) \cap E(T_2)| = 0$, 
%
$|E(T_1) \cup E(T_2)| = |V(S)| - 1+ |V(S')| - 1 = n - 2$.
%
Each such pair $(T_1, T_2)$ is a spanning forest of $n - 2$ edges. 
Given $i$ is the root of $T_1$ in $S$, we can choose $|V(S')|$ roots for 
$T_2$ in $S'$. There being $|\mathcal{T}_S| ~ |\mathcal{T}_{S'}|$ 
such pairs:
$\varepsilon(\mathcal{F}^{ii}_{n - 2|P}) = |\mathcal{T}_S| ~ |\mathcal{T}_{S'}| ~ |V(S')|$.
%

\noindent $\square$
%

\noindent By symmetry, for $j \in V(S'):$
$$\varepsilon(\mathcal{F}^{jj}_{n - 2|P}) = |\mathcal{T}_S| ~ |\mathcal{T}_{S'}| ~ |V(S)|$$
%  
\begin{mylem}
\label{lem:RandEccAllPartitions}
%
Given $\mathcal{P}(G)$, the set of all bi-partitions of $G$: 
%
$$\varepsilon(\mathcal{F}^{ii}_{n-2}) = \sum_{P \in \mathcal{P}(G)}^{i \in V(S)} |\mathcal{T}(S)| |\mathcal{T}(S')| |V(S')|$$
%
\end{mylem}
%
\textbf{Proof:} By definition, $\forall F \in \mathcal{F}_{n-2}$, 
$F$ belongs to exactly one of the partitions of $G$. Hence, 
%
$\mathcal{F}^{ii}_{n-2} = \coprod_{P \in \mathcal{P}}  \varepsilon(\mathcal{F}^{ii}_{n - 2|P})$.
%
As the RHS is a disjoint union, counting members on both sides we obtain the proof.
%

\noindent $\square$
%

\noindent Evidently, combining the results of the two lemmas above, we obtain the proof for 
Theorem \ref{thm:LpPropPartitions}.

\noindent $\square$
%

\noindent To paraphrase, given a bi-partition $P=(S, S') \in \mathcal{P}(G)$, such that $i \in V(S)$ 
and $j \in |V(S')|$, Lemma \ref{lem:RandEccPerPartition} yields:  
$\varepsilon(\mathcal{F}^{ii}_{n - 2|P})/\varepsilon(\mathcal{F}^{jj}_{n - 2|P}) = |V(S')|/|V(S)|$. 
%
Clearly, for a given bi-partition, nodes in the larger of the two components of $P$ have a 
lower number of spanning forests rooted at them than those in the smaller component and vice versa. 
By extension, 
%
\begin{eqnarray*}
%
  l^{+}_{ii} - l^{+}_{jj} 
 &\propto& \sum_{P \in \mathcal{P}(G)}^{i \in V(S), j \in V(S')} |\mathcal{T}(S)| |\mathcal{T}(S')| (|V(S')| - |V(S)|)
 %
\label{equ:PropLpForest}
%
\end{eqnarray*}
%
can be interpreted as a comparative measure of connectedness of nodes $i$ and $j$. Note that 
for $P \in \mathcal{P}(G)$, the RHS of (\ref{equ:PropLpForest}) is zero when nodes $i$ and $j$ belong 
to the same component of $P$ or if $|V(S)| = |V(S')|$ and positive when 
$i \in V(S), j \in V(S')$ and $|V(S')| > |V(S)|$ or vice versa. 
%
Therefore,  a node $i$ with higher structural centrality stays connected to 
a greater number of nodes on an average in a disconnected network, than one with lower 
structural centrality and is consequently more immune to random edge failures in the network.

By simple extension, Kirchoff index represents the average connectedness of all the nodes 
when a failure of a subset of edges partitions the network into two halves, thereby truly reflecting 
overall network robustness. It is easy to demonstrate that of all trees of order $n$, the star has the 
lowest Kirchoff index and the root of the star has highest $\mathcal{C}^*(i)$ value. Also, amongst all 
graphs of order $n$ with differing volumes, the completely connected graph $K_n$ has the lowest 
Kirchoff index. 
%
%#################
%
% ----- End Section -----
%
%#################
%

==> Section_6_Empirical.tex <==
%%%%%%%%
%
% --- Section ---
%
%%%%%%%%
%
%
\begin{figure*}[t]
\centerline{\begin{tabular}{ccc}
\scalebox{0.8}{\includegraphics[width = 90mm]{graph_Abilene.eps}}
&
\scalebox{0.9}{\includegraphics[width = 60mm]{graph_Top_Low.eps}}
&
\scalebox{0.65}{\includegraphics[width = 50mm]{graph_Perturb_Top_Higher_Stat.eps}}
\\
(a) Abilene Topology & (b) Simulated topology & (c) Perturbations
%
\end{tabular}}
\caption{Abilene Network and a simulated topology.}
\label{fig:AbileneTop}
\end{figure*}
%
%
\begin{figure*}[h]
\centerline{\begin{tabular}{c}
%
\scalebox{0.9}{\includegraphics[width = 180mm]{plot_Comp_Top_Low_SC_GC_SC_65.eps}}
%
\end{tabular}}
\caption{Max-normalized centralities for simulated topology.}
\label{fig:plotTopNets}
\end{figure*}
%
%
We now empirically study the properties of structural centrality $(\mathcal{C}^*(i))$ and 
Kirchoff index (we use $\mathcal{K}^* = \mathcal{K}^{-1}$ henceforth to maintain {\em higher is better}). 
We first show in \textsection\ref{subSec:StructRoles}, how a rank-order of nodes in terms of their structural centralities 
captures their structural roles in the network and then in  \textsection\ref{subSec:Sensitivity} demonstrate how it, 
along with Kirchoff index, is appropriately sensitivity to rewirings and local perturbations in the network.
%
%%%%%%%%%%
% --- Subsection ---
%%%%%%%%%%
%
\subsection{Identifying Structural Roles of Nodes}
\label{subSec:StructRoles}
%
%
Consider the router level topology of the Abilene network 
(Fig. \ref{fig:AbileneTop}(a)) \cite{Abilene}. At the core of this topology, 
is a ring of $11$ POP's, spread across mainland US, through which 
several networks interconnect. Clearly, the connectedness of such a 
network is dependent heavily on the low degree nodes on the ring. 
For illustration, we mimic the Abilene topology, with a simulated network 
(Fig. \ref{fig:AbileneTop}(b)) which has a 4-node core $\{v_1,...,v_4\}$ 
that connects $10$ networks through gateway nodes $\{v_5,...,v_{14}\}$ 
(Fig.\ref{fig:AbileneTop}(b)). 
%

Fig. \ref{fig:plotTopNets} shows the (max-normalized) values of geodesic closeness $(GC)$, 
subgraph centrality $(SC)$ and structural centrality $\mathcal{C}^*$ for the core $\{v_1,...,v_4\}$, 
gateway $\{v_5,...,v_{14}\}$ and other nodes $\{v_{15},...,v_{65}\}$ in topology (Fig.\ref{fig:AbileneTop}(b)). 
Notice that $v_5$ and $v_6$, two of the gateway nodes in the topology, have the highest values of degree
in the network i.e. $(d(v_5)=d(v_6)=10)$ while $v_{14}$ has the highest subgraph centrality $(SC)$. 
%
In contrast, $\mathcal{C}^*(i)$ ranks the four core nodes higher 
than all the gateway nodes with $v_1$ at the top. The relative peripherality 
of $v_5, v_6$ and  $v_{14}$ as compared to the core nodes requires no 
elaboration. As far as geodesic centrality $(GC)$ is concerned, it ranks all the nodes in the subnetwork 
abstracted by $v_{5}$, namely $v_{15}-v_{23}$, as equals even though $v_{22}$ and $v_{23}$ have 
redundant connectivity to the network through each other and are, ever so slightly, better connected than 
the others - a property reflected in their $\mathcal{C}^*(i)$ rankings. 
%

We see similar characterization of structural roles of nodes in two real world networks in terms of structural centrality: 
the western states power-grid network \cite{Watts98} and a social network of co-authorships 
\cite{Newman06}, as shown through a color scheme based on $\mathcal{C}^*(i)$ 
values in Fig. \ref{fig:RealWorldNets}. Core-nodes connecting different sub-communities of 
nodes in both these real world networks are recognized effectively by structural centrality 
as being more central ($Red$ end of the spectrum) than several higher degree peripheral nodes.
%
%
\begin{figure*}[ht]
\centerline{\begin{tabular}{cc}
%
\scalebox{0.7}{\includegraphics[width = 90mm, angle=90]{graph_PowerGrid.eps}}
%
&
%
\scalebox{0.7}{\includegraphics[width = 70mm, angle=90]{graph_NetScience_Coauthorships.eps}}
%
\\
%
(a) The western-states power grid network \cite{Watts98}
%
&
%
(b) A network of co-authorships in network sciences \cite{Newman06}
%
\end{tabular}}
\caption{Real world networks: $Red \rightarrow Turqoise$ in order of decreasing $\mathcal{C}^*(i)$.}
\label{fig:RealWorldNets}
\end{figure*}
%
%
\
%
%%%%%%%%%%
% --- Subsection ---
%%%%%%%%%%
%
\subsection{Sensitivity to Local Perturbations}
\label{subSec:Sensitivity}
%
%
\begin{figure*}[ht]
\centerline{\begin{tabular}{cc}
%
\scalebox{0.8}{\includegraphics[width = 110mm]{plot_Comp_Top_High_SC_GC_SC_23.eps}}
&
\scalebox{0.8}{\includegraphics[width = 110mm]{plot_Comp_Top_Stat_SC_GC_SC_23.eps}}
\\
(a) After PERT-I & (b) After PERT-II
%
\end{tabular}}
\caption{Max-normalized values of structural centrality, geodesic closeness and subgraph centrality for core, gateway and some other nodes.}
\label{fig:plotTopNets_HighStat_SC_GC_SC}
\end{figure*}
%
%
An important property of centrality measures is their sensitivity to perturbations in 
network structure. 
%
Traditionally, structural properties in real world networks have been equated to 
average statistical properties like power-law/scale-free degree distributions and 
rich club connectivity \cite{Barabasi00, Faloutsos99, Barabasi01}.  
However, the same degree sequence $D = \{d(1)\geq d(2)\geq ...\geq d(n)\}$, 
can result in graphs of significantly varying topologies. 
Let $\mathcal{G}(D)$ be the set of all connected graphs with scaling 
sequence $D$. The generalized Randic index $R_1(G)$ 
\cite{BollobasErdos98, Randic75}:
%
\begin{equation}
%
R_1(G) = \sum_{e_{ij} \in E(G)} d(i) d(j) \label{equ:S-Fact}
%
\end{equation}
%
%
where $G \in \mathcal{G}(D)$, is  considered to be a measure of overall 
connectedness of $G$. Higher $R_1(G)$ suggests that nodes of higher degrees 
connect with each other with high probability thereby displaying the so-called 
{\em rich club connectivity} (RCC) in $G$ \cite{LiAldersonWillingerDoyle04}. 
Similarly, the average of each centrality/betweenness index 
($GC, SC, GB, RB$ averaged over the set of nodes), is in itself a global structural 
descriptor for the graph $G$ \cite{Estrada05}. 
%
We now examine the sensitivity of each index with respect to local perturbations 
in the subnetwork abstracted by the core node $v_1$ and its two gateway neighbors 
$v_5$ and $v_6$.   
%

First, we rewire edges $e_{15,5}$ and $e_{6,1}$ to $e_{15,1}$ and $e_{6,5}$ 
respectively (PERT-I Fig. \ref{fig:AbileneTop}(c)). PERT-I is a degree  
preserving rewiring which only alters local connectivities i.e. neither individual node degrees 
nor average node degree changes.
% 
Fig. \ref{fig:plotTopNets_HighStat_SC_GC_SC}(a) and Fig. \ref{fig:plotTopNets_HighStat_SC_GB_RB} 
respectively show the altered values of centralities $(\mathcal{C}^*, GC, SC)$ and 
betweennesses, geodesic and random-walk i.e. $(GB, RB)$, after PERT-I.
% 
Note, after  PERT-I,  $v_{15}$ is directly connected to $v_1$ which makes $\mathcal{C}^*(v_{15})$ 
comparable to other gateway nodes while $SC(v_{15}), GB(v_{15}), RB(v_{15})$ seem to be entirely 
unaffected.
% 
Moreover, PERT-I also results in $v_6$ losing its direct link to the core, reflected in the 
decrease in $\mathcal{C}^*(v_6)$ and a corresponding increase in $\mathcal{C}^*(v_5)$. 
$\mathcal{C}^*(i)$, however, still ranks the core nodes higher than $v_5$ 
(whereas $SC, GB, RB$ do not) because PERT-I being a local perturbation should not affect 
nodes outside the sub-network --- 
$v_1$ continues to abstract the same sub-networks from the rest of the 
topology. We, therefore, observe that $\mathcal{C}^*(i)$ is appropriately 
sensitive to the changes in connectedness of nodes in the event of local 
perturbations.  But what about the network on a whole?
% 
%
\begin{figure}[ht]
\centerline{\begin{tabular}{c}
%
\scalebox{0.8}{\includegraphics[width = 110mm]{plot_Comp_Top_High_SC_GB_RB_23.eps}}
%
\end{tabular}}
\caption{After PERT-I: Max-normalized values of structural centrality, geodesic and random-walk betweennesses for core, gateway and some other nodes.}
\label{fig:plotTopNets_HighStat_SC_GB_RB}
\end{figure}
%
%
\begin{table}[t]
%
\caption{Sensitivity to local perturbations, 
$\overline{X} = 1/n \sum_i^n X(i)$: Avg. node centrality for a network.}
% 
\label{Tab:Sensitivity_To_Pert}
\begin{center}
\small
\begin{tabular}{||l|l||c|c||}
\hline
$\#$ & Structural Descriptor & PERT-I  & PERT-II \\
\hline\hline
1 & $\mathcal{K}^*(G)$ (or $\overline{\mathcal{C}^*}$) & $\downarrow$ & $\uparrow$ \\
%
\hline
%
2 & $R_1(G)$ & $\uparrow$ & $\leftrightarrow$ \\
%
\hline
%
3 & $\overline{GC}$ & $\downarrow$ & $\uparrow$ \\
%
\hline
%
4 & $\overline{SC}$, $\overline{GB}$  & $\uparrow$ & $\downarrow$ \\
%
\hline
%
5 & $\overline{RB}$ & $\uparrow$ & $\uparrow$ \\
%
\hline
%
\end{tabular}
\end{center}
\end{table}
%

%
Let $G$ and $G_1$ be the topologies before and after PERT-I. $G_1$ is less 
well connected overall than $G$  as the failure of $e_{5,1}$ in $G_1$ 
disconnects $19$ nodes from the rest of the network as compared to $10$ nodes 
in $G$. However,
%
$$\Delta R_1(G \rightarrow G_1) = \frac{R_1(G_1) - R_1(G)} {R_1(G)} = 0.029$$ 
%
as the two highest degree nodes ($v_5$ and $v_6$) are directly connected in 
$G_1$ (see TABLE \ref{Tab:Sensitivity_To_Pert} for the sensitivity of other centrality based 
global structural descriptors).
% 
In contrast, $\Delta \mathcal{K}^*(G \rightarrow G_1) = -0.045$, which rightly  
reflects the depreciation in overall connectedness after PERT-I 
(recall  $\mathcal{K}^*(G) =  \mathcal{K}^{-1}(G$). 
Table \ref{Tab:Sensitivity_To_Pert} shows the changes in the average of all centrality and 
betweenness indices post PERT-I. 
%

A subsequent degree preserving perturbation PERT-II of $G_1$, 
rewiring $e_{22,23}$ and $e_{24,25}$ to $e_{22,25}$ and $e_{23,24}$,
to obtain $G_2$, creates two cycles in $G_2$ that safeguard against the failure 
of edge $e_{5,6}$. This significantly improves local connectivities in the sub-network.  
However, $\Delta R_1(G_1 \rightarrow G_2) = 0$ (and average $SC$ decreases) 
while $\Delta \mathcal{K}^*(G_1 \rightarrow G_2) = 0.036$ which once again shows 
the efficacy of Kirchoff index as a measure of global connectedness of networks.
%
%
%%%%%%%%%%%
%
% --- End Section ---
%
%%%%%%%%%%%

